Verifying Deep Learning-based Decisions for Facial Expression Recognition

Neural networks with high performance can still be biased towards non-relevant features. However, reliability and robustness is especially important for high-risk fields such as clinical pain treatment. We therefore propose a verification pipeline, which consists of three steps. First, we classify facial expressions with a neural network. Next, we apply layer-wise relevance propagation to create pixel-based explanations. Finally, we quantify these visual explanations based on a bounding-box method with respect to facial regions. Although our results show that the neural network achieves state-of-the-art results, the evaluation of the visual explanations reveals that relevant facial regions may not be considered.

==> eval.tex <==
\section{Evaluation}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}\hline
AUs & \multicolumn{2}{|c|}{Actor Study} & \multicolumn{2}{|c|}{CK+} & \multicolumn{2}{|c|}{UNBC}\\ 
\hline
& $\mu$ & $\mu_{w}$ & $\mu$ & $\mu_{w}$ & $\mu$ & $\mu_{w}$ \\ 
\hline
AU04 & 0.504 & 0.969 & 0.554 & 1.022 & 0.587 & 1.095\\ 
AU06 & 0.42 & 0.808 & 0.475 & 0.873 & 0.579 & 1.04\\ 
AU07 & 0.43 & 0.833 & 0.52 & 0.954 & 0.532 & 0.957\\ 
AU09 & 0.366 & 0.649 & 0.736 & 1.276 & 0.695 & 1.183\\ 
AU10 & 0.204 & 0.599 & 0.516 & 1.445 & 0.336 & 0.796\\ 
AU25 & 0.466 & 1.174 & 0.35 & 0.997 & 0.286 & 0.823\\ 
AU26 & 0.488 & 1.228 & 0.326 & 0.933 & 0.312 & 0.915\\ 
AU27 & 0.484 & 1.218 & 0.341 & 0.973 & 0.475 & 1.212\\ 
\hline
\end{tabular}
 \caption{Complete}
 \end{table}
 
 \begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}\hline
AUs & \multicolumn{2}{|c|}{Actor Study} & \multicolumn{2}{|c|}{CK+} & \multicolumn{2}{|c|}{UNBC}\\ 
\hline
& $\mu$ & $\mu_{w}$ & $\mu$ & $\mu_{w}$ & $\mu$ & $\mu_{w}$ \\ 
\hline
AU04 & 0.391 & 0.752 & 0.563 & 1.037 & 0.671 & 1.251\\ 
AU06 & 0.318 & 0.613 & 0.474 & 0.872 & 0.616 & 1.107\\ 
AU07 & 0.296 & 0.576 & 0.535 & 0.981 & 0.523 & 0.936\\ 
AU09 & 0.254 & 0.45 & 0.805 & 1.399 & 0.798 & 1.361\\ 
AU10 & 0.213 & 0.611 & 0.556 & 1.549 & 0.326 & 0.774\\ 
AU25 & 0.561 & 1.418 & 0.347 & 0.986 & 0.243 & 0.701\\ 
AU26 & 0.609 & 1.535 & 0.344 & 0.985 & 0.27 & 0.788\\ 
AU27 & 0.655 & 1.65 & 0.341 & 0.964 & 0.456 & 1.139\\ 
 \hline
\end{tabular}
 \caption{Top25}
 \end{table}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline
AUs & \multicolumn{3}{|c|}{Actor Study} & \multicolumn{3}{|c|}{CK+} & \multicolumn{3}{|c|}{UNBC}\\ 
\hline
& $\mu$ & $\mu_{w}$ & n & $\mu$ & $\mu_{w}$ & n & $\mu$ & $\mu_{w}$ & n\\ 
\hline
AU04 & 0.503 & 0.97 & 11249 & 0.554 & 1.022 & 3753 & 0.497 & 0.934 & 291\\ 
AU06 & 0.417 & 0.802 & 6887 & 0.475 & 0.873 & 2174 & 0.503 & 0.892 & 1740\\ 
AU07 & 0.429 & 0.832 & 13098 & 0.52 & 0.954 & 2222 & 0.568 & 1.003 & 1439\\ 
AU09 & 0.363 & 0.644 & 3363 & 0.736 & 1.276 & 1191 & 0.689 & 1.153 & 213\\ 
AU10 & 0.204 & 0.599 & 3143 & 0.516 & 1.445 & 383 & 0.441 & 1.071 & 7\\ 
AU25 & 0.466 & 1.175 & 13497 & 0.35 & 0.997 & 5358 & 0.354 & 0.979 & 738\\ 
AU26 & 0.49 & 1.234 & 7537 & 0.326 & 0.933 & 882 & 0.197 & 0.583 & 33\\ 
AU27 & 0.486 & 1.224 & 1214 & 0.341 & 0.973 & 1285 & 0.0 & 0.0 & 1\\ 
\hline
 \end{tabular}
 \caption{Standard, only correct prediction}
 \end{table}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline
AUs & \multicolumn{3}{|c|}{Actor Study} & \multicolumn{3}{|c|}{CK+} & \multicolumn{3}{|c|}{UNBC}\\ 
\hline
& $\mu$ & $\mu_{w}$ & n & $\mu$ & $\mu_{w}$ & n & $\mu$ & $\mu_{w}$ & n\\ 
\hline
AU04 & 0.39 & 0.752 & 11249 & 0.563 & 1.037 & 3753 & 0.588 & 1.103 & 291\\ 
AU06 & 0.311 & 0.6 & 6887 & 0.474 & 0.872 & 2174 & 0.471 & 0.835 & 1740\\ 
AU07 & 0.295 & 0.574 & 13098 & 0.535 & 0.981 & 2222 & 0.553 & 0.972 & 1439\\ 
AU09 & 0.248 & 0.44 & 3363 & 0.805 & 1.399 & 1191 & 0.733 & 1.226 & 213\\ 
AU10 & 0.214 & 0.611 & 3143 & 0.556 & 1.549 & 383 & 0.563 & 1.362 & 7\\ 
AU25 & 0.562 & 1.42 & 13497 & 0.347 & 0.986 & 5358 & 0.245 & 0.669 & 738\\ 
AU26 & 0.613 & 1.546 & 7537 & 0.344 & 0.985 & 882 & 0.118 & 0.315 & 33\\ 
AU27 & 0.661 & 1.664 & 1214 & 0.341 & 0.965 & 1285 & 0.0 & 0.0 & 1\\ 
\hline
 \end{tabular}
 \caption{top25, only correct prediction}
 \end{table}
 
%\begin{figure}[h]
%	\includegraphics[width=\textwidth]{images/dummy_pic.png}
%	\caption{Dummy Figure}
%	\label{fig:heatmaps}
%\end{figure}
